Evolution and The Knightian Blindspot of Machine Learning

This paper claims that machine learning (ML) largely overlooks an important facet of general intelligence: robustness to a qualitatively unknown future in an open world. Such robustness relates to Knightian uncertainty (KU) in economics, i.e. uncertainty that cannot be quantified, which is excluded from consideration in ML's key formalisms. This paper aims to identify this blind spot, argue its importance, and catalyze research into addressing it, which we believe is necessary to create truly robust open-world AI. To help illuminate the blind spot, we contrast one area of ML, reinforcement learning (RL), with the process of biological evolution. Despite staggering ongoing progress, RL still struggles in open-world situations, often failing under unforeseen situations. For example, the idea of zero-shot transferring a self-driving car policy trained only in the US to the UK currently seems exceedingly ambitious. In dramatic contrast, biological evolution routinely produces agents that thrive within an open world, sometimes even to situations that are remarkably out-of-distribution (e.g. invasive species; or humans, who do undertake such zero-shot international driving). Interestingly, evolution achieves such robustness without explicit theory, formalisms, or mathematical gradients. We explore the assumptions underlying RL's typical formalisms, showing how they limit RL's engagement with the unknown unknowns characteristic of an ever-changing complex world. Further, we identify mechanisms through which evolutionary processes foster robustness to novel and unpredictable challenges, and discuss potential pathways to algorithmically embody them. The conclusion is that the intriguing remaining fragility of ML may result from blind spots in its formalisms, and that significant gains may result from direct confrontation with the challenge of KU.

==> bkup/name.tex <==
\begin{comment}
\subsection{The Promise of KU-Capable Simulators}

Training ML systems sometimes entails training the ML system in a virtual simulation that attempts to mimic certain aspects of reality - typical in the development of ML methods for robotics for example. The hope is that in mimicking those aspects, the ML model can “transfer” its knowledge accordingly, once placed into a robot in the real world. (Also known as the “sim2real” problem). Leaving aside the quality of simulations of the real world, (a complex endeavor in and of itself) - and even a completely successful sim2real transfer, typical simulators leave aside and ignore one of the most important aspects of reality: That it is open-ended, and subject to Knightian Uncertainty (KU). As we have seen, natural systems have not only been successful at performing their normative tasks required for survival, but are also adept at dealing with environments subject to KU - a facet missing from current simulations for robotics. Hence, the quality that really matters in preparing ML methods - especially ones destined for interaction with the real world - is not so much reflecting particular physical attributes of reality per se, but in mimicking the continuing presence of unknown unknowns. In other words, resiliency to unknown unknowns isn’t about adapting to what can be predicted, but in adapting to what can’t be predicted - contending with qualitatively different scenarios that the agent has no way of knowing beforehand. (As an analogy, what might happen if some rules in the game of chess were to suddenly change during the game - or more to the point - a new cast of pieces with their own capabilities were to suddenly appear). 

\subsection{The Promise KU-Capable Systems and KU-Growing AIs:}

While traditional ML attempts to handcraft the tasks, the learning algorithms, the datasets, the benchmarks, the objectives and the architectures - those all are up for grabs in natural evolution, and the lines between them are blurred. It seems like radical persistence and thriving in the face of KU may well be the ultimate singular (and sparsest condition), that yields winning combinations of the above that marvel or go above and beyond our current capabilities - in non-trivial ways that humans cannot possibly conceive of. 

Some examples of KU-capable systems in nature - and in neuroscience in particular - point to sensorimotor programs and sensorimotor program synthesis as examples of systems that have developed in nature which allow animals a KU-resilience that marvels what can be accomplished by our best robotic systems today - solutions to Moravec's paradox - the holy grail in “Physical AI” today. To be sure, they need not be the only ones, but they are notable in their own right. In many ways, robotics today suffers from being unable to adapt to KU-situations, with massive safety and resiliency repercussions across various swaths of industries.

Insights from KU-solutions in nature, the processes that lead to KU-resiliency, married with the trajectory of compute, and open-ended generative modelling, might offer a way to develop AI-GAs that develop KU-capable systems at rate and quality that marvels what humans can come up with. 


\end{comment}
